SnipGen: A Mining Repository Framework for Evaluating LLMs for Code

Language Models (LLMs), such as transformer-based neural networks trained on billions of parameters, have become increasingly prevalent in software engineering (SE). These models, trained on extensive datasets that include code repositories, exhibit remarkable capabilities for SE tasks. However, evaluating their effectiveness poses significant challenges, primarily due to the potential overlap between the datasets used for training and those employed for evaluation. To address this issue, we introduce SnipGen, a comprehensive repository mining framework designed to leverage prompt engineering across various downstream tasks for code generation. SnipGen aims to mitigate data contamination by generating robust testbeds and crafting tailored data points to assist researchers and practitioners in evaluating LLMs for code-related tasks. In our exploratory study, SnipGen mined approximately 227K data points from 338K recent code changes in GitHub commits, focusing on method-level granularity. SnipGen features a collection of prompt templates that can be combined to create a Chain-of-Thought-like sequence of prompts, enabling a nuanced assessment of LLMs' code generation quality. By providing the mining tool, the methodology, and the dataset, SnipGen empowers researchers and practitioners to rigorously evaluate and interpret LLMs' performance in software engineering contexts.

==> bk/dataset.tex <==
\section{Experience Report}\label{sec:experience}


\subsection{Collecting Code Samples}
\input{tabs/dedupe}

As represented in the first step of the pipeline (refer to Fig.~\ref{fig:collection}-\circled{1}),  we filtered the most popular Python Github repositories using the following query: $language:Python$, $fork:false$, $size:>=30,000$,  $pushed:>2021-12-31$, $stars:>1,000$.

Our dataset aims to avoid data snooping, a problem where training samples are wrongly used to test statistical hypotheses. To do this, we focused on collecting code changes only up to January 2022. This is because we hypothesize \chatgpt and most newer \llms have not been trained on commits made after January 2, 2022, according to \cite{openai2023gpt4}. We carefully selected new methods from each commit, resulting in about 338K data points. For each of these data points, we extracted the comments or any associated documentation that describes its functionality.

In the second step (Fig.~\ref{fig:collection}-\circled{2}), we engineered and pre-processed code and documentation-related and security weaknesses from collected data points. We parsed the AST variables for our data points by employing the Tree-Sitter library. Therefore, each data point encompasses the \textit{code} and related features from the AST analysis. The AST features numerically describe the \ASTerrors, \ASTlevels, and \ASTnodes. The AST also describes the structural shape for the \textit{code} introducing the \textit{n\_words}, \textit{vocab\_size}, \tokenCount, and \whitespaces. The vocabulary size measures the count of unique words without repetition. \tokenCount is determined by using a universal tokenizer. We also calculated the number of variables that the \textit{code} is using and it is reflected as \identifiers. As for determining the security weaknesses, we use codeQL scanning suite \cite{noauthor_codeql_nodate}, focussing on the top `25'  Common Weakness Enumeration (CWE) \cite{noauthor_cwe_nodate}. CodeQL identifies vulnerability issues by scanning for predetermined rules defined with its query language. We report CodeQL results with the span positions of the identified vulnerability in the code. 

To guarantee efficient data management, we stored raw and preprocessed data points in a relational database once the previous features were engineered and extracted. Next, we removed duplicated samples using a distinct query reducing the testbed size to $\approx 227K$ data points for code. Of these reduced data points, $\approx 77K$ contains a valid \docstring. A \docstring is valid when its text is larger than 3 words. We use \textit{CLD3} library to detect the \textit{language} for each \docstring with a threshold of 0.9 to define sentence language such as English, Chinese, Spanish, etc.
Once these features were computed, the raw data was stored in a relational database, enabling efficient management and summarization of many data points.


In the third step \ref{fig:collection}-\circled{3}), we manually verified $960$ out of $\approx 227K$ data points. These verified data points were randomly selected from \textit{RawData} and \textit{RawDataDocstring} for a manual evaluation. The remaining data points underwent automatic validation. Our validation process ensures that the date of each pushed commit falls within the range of dates stated in the original query. Additionally, we confirmed that the methods associated with each commit were indeed updated within the same date range. Furthermore, we assessed the meaningfulness of the \docstring and \commitMessage by scrutinizing the consistency of the natural language descriptions with the actual code implementation, resulting in the removal of $\approx1.9\%$ from \textit{RawDataDocstring} and obtaining $\approx57K$ datapoints. Finally, \complexity was validated using the Codalyze plugin in Visual Studio Code.

In the final step (Fig.\ref{fig:collection}-\circled{4}), we sampled until $5k$ data points from the \textit{RawData} testbed to construct six additional testbeds, each tailored for a specific SE task. \snipgen encompasses \randomCut, \withDocstring, and \fromDocstring for \textit{code completion}; \commitGen for \textit{code generation}; \summarizationGen for \textit{code summarization}; and \textit{VulnerabilitySpan} for vulnerability detection. Details about these supplementary testbeds are outlined in Tab.~\ref{tab:dedupe}.

To create \randomCut, we selected data points with more than $10$ tokens or $100$ characters, and subsequently, each data point was randomly truncated after the method signature. For \summarizationGen and \commitGen, we filtered \textit{RawDataDocstring} data points with more than 10 words or 50 characters. After establishing the five testbeds, we employed Jaccard similarity on preprocessed data points with the BPE HuggingFace tokenizer to eliminate duplicate snippets. Given the absence of de-duplication between training and test sets (i.e., no multiset threshold), we configured a $0.7$ similarity threshold for our testbeds \cite{Allamanis19, wang_neural_2019}. Table.~\ref{tab:dedupe} provides information about the SE task associated with each curated testbed, the percentage of detected duplicates, final size and generated number of prompts.




 %Our methodology depicts data extraction based on experiment-specific parameters. Researchers are afforded the flexibility to choose datasets that align most seamlessly with their objectives. The pivotal role of \snipgen comes into play as it adeptly collects and extracts features from the chosen data. Each snippet is systematically labeled according to its relevance to a specific code generation sub-task in software engineering (SE). The presence of a \docstring within a snippet is leveraged by \snipgen to incorporate textual context seamlessly. Subsequently, a prompt template is strategically selected based on the SE sub-task, and a prompt is dynamically generated. This prompt serves as an invaluable tool for evaluating Language Model for Code (LLMc) but can also be efficiently trained and tested on canonical datasets, ensuring robustness and adaptability in the ever-evolving landscape of code generation research.


==> tabs/design_1_models.tex <==
\begin{table}[h]
\centering
\caption{Large Language Models characteristics.}
\vspace{-0.2cm}
\label{tab:models}

\scalebox{0.8}{%
\setlength{\tabcolsep}{5pt} 

%%%%%%%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lllll}
\hline
\multicolumn{5}{c}{\textbf{Large Language Models (LLMs)}} \\ \hline
\multicolumn{1}{c}{\textit{Type}} & \textit{LLMs} & \multicolumn{1}{c}{\textit{Name}} & \multicolumn{1}{c}{\textit{Architecture}} & \multicolumn{1}{c}{\textit{Size}} \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Natural L.\\ gpt-3\end{tabular}}} & M1 & gpt-neo-125m & \textit{gpt-3} & 125M \\
 & M2 & gpt-neo-1.3B & \textit{gpt-3} & 1.3B \\
 & M3 & gpt-neo-2.7B & \textit{gpt-3} & 2.7B \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Natural L.\\ codegen\end{tabular}}} & M4 & codegen-350M-nl & \textit{codegen} & 350M \\
 & M5 & codegen-2B-nl & \textit{codegen} & 2B \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Multi-\\ Language\end{tabular}}} & M6 & codeparrot-small-multi & \textit{gpt-2} & 110M \\
 & M7 & codegen-350M-multi & \textit{codegen-350M-nl} & 350M \\
 & M8 & codegen-2B-multi & \textit{codegen-2B-nl} & 2B \\ \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mono-\\ Language\end{tabular}}} & M9 & codeparrot-small & \textit{gpt-2} & 110M \\
 & M10 & codeparrot & \textit{gpt-2} & 1.5B \\
 & M11 & codegen-350M-mono & \textit{codegen-350M-multi} & 350M \\
 & M12 & codegen-2B-mono & \textit{codegen-2B-multi} & 2B \\ \hline
\end{tabular}


%%%%%%%%%%%%%%%%%%
}


%\vspace{-0.45cm}

\end{table}

==> tabs/design_2_models_performance.tex <==
\begin{table*}[h]
\centering
\caption{Syntax Concept Empirical Evaluation Results (bold: best, underlined: worst). }
\vspace{-0.2cm}
\label{tab:models_performance}

\scalebox{0.85}{%
\setlength{\tabcolsep}{5pt} 

%%%%%%%%%%%%%%%%%

\begin{tabular}{llclccclcccccccccc}
\hline
\multicolumn{1}{c}{} &  &  &  & \multicolumn{3}{c}{\textbf{Canonical Score}} &  & \multicolumn{10}{c}{\textbf{Interpretable Score}} \\ \cline{5-7} \cline{9-18} 
\multicolumn{1}{c}{} &  &  &  & \multicolumn{2}{c}{\textbf{Extrinsic}} & \multicolumn{1}{l}{\textbf{Intrinsic}} &  & \multicolumn{10}{c}{\textbf{Syntax-Interpretable Performance (bootstrapped median)}} \\ \cline{5-7} \cline{9-18} 
\multicolumn{1}{c}{\multirow{-3}{*}{\textbf{Types}}} &  & \multirow{-3}{*}{\textbf{LLMs}} &  & \multicolumn{1}{l}{\textit{BLEU-4}} & \multicolumn{1}{l}{\textit{CodeBLEU}} & ACC. & \textit{} & \multicolumn{1}{l}{\textit{Data Str.}} & \multicolumn{1}{l}{\textit{Decision}} & \multicolumn{1}{l}{\textit{Except.}} & \multicolumn{1}{l}{\textit{F. Prog.}} & \multicolumn{1}{l}{\textit{Iter.}} & \multicolumn{1}{l}{\textit{NL}} & \multicolumn{1}{l}{\textit{Oper.}} & \multicolumn{1}{l}{\textit{Scope}} & \multicolumn{1}{l}{\textit{Testing}} & \multicolumn{1}{l}{\textit{Types}} \\ \hline
 &  & \textit{M1} &  & 0.013 & 0.139 & 0.48 &  & 0.50 & 0.52 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.43}} & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.49}} & 0.74 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.32}} & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.48}} & 0.51 & 0.59 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.33}} \\
 &  & \textit{M2} &  & 0.016 & 0.151 & 0.59 &  & 0.60 & 0.61 & 0.53 & 0.62 & 0.79 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.43}} & 0.57 & 0.68 & 0.68 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.44}} \\
\multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Natural L.\\ GPT-3\end{tabular}}} &  & \textit{M3} &  & 0.015 & 0.163 & \textbf{0.62} &  & 0.62 & 0.63 & 0.56 & 0.66 & \cellcolor[HTML]{CACDFA}\textbf{0.81} & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.46}} & 0.60 & 0.74 & 0.70 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.47}} \\ \hline
 &  & \textit{M4} &  & 0.015 & 0.151 & 0.55 &  & 0.56 & 0.57 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.45}} & 0.57 & 0.77 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.39}} & 0.54 & 0.64 & 0.64 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.40}} \\
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Natural L.\\ Codegen\end{tabular}}} &  & \textit{M5} &  & 0.016 & 0.155 & \textbf{0.65} &  & 0.65 & 0.65 & 0.58 & 0.68 & \cellcolor[HTML]{CACDFA}\textbf{0.82} & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.48}} & 0.61 & 0.78 & 0.72 & 0.50 \\ \hline
 &  & \textit{M6} &  & 0.010 & 0.189 & 0.57 &  & 0.54 & 0.55 & 0.64 & 0.60 & 0.60 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.40}} & 0.54 & 0.71 & 0.67 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.42}} \\
 &  & \textit{M7} &  & 0.015 & 0.171 & 0.68 &  & 0.63 & 0.72 & 0.75 & 0.70 & 0.69 & 0.51 & 0.62 & 0.83 & 0.73 & 0.51 \\
\multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Multi-\\ Language\end{tabular}}} &  & \textit{M8} &  & 0.016 & 0.177 & \textbf{0.79} &  & 0.74 & 0.79 & \cellcolor[HTML]{CACDFA}\textbf{0.83} & 0.81 & 0.77 & 0.65 & 0.74 & \cellcolor[HTML]{CACDFA}\textbf{0.91} & 0.80 & 0.71 \\ \hline
 &  & \textit{M9} &  & 0.011 & 0.194 & 0.61 &  & 0.58 & 0.58 & 0.68 & 0.66 & 0.63 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.46}} & 0.57 & 0.73 & 0.69 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} {\ul 0.47}} \\
 &  & \textit{M10} &  & 0.011 & 0.196 & 0.71 &  & 0.67 & 0.67 & \cellcolor[HTML]{CACDFA}\textbf{0.80} & 0.76 & 0.70 & 0.59 & 0.66 & \cellcolor[HTML]{CACDFA}\textbf{0.82} & 0.74 & 0.64 \\
 &  & \textit{M11} &  & 0.014 & 0.179 & 0.73 &  & 0.68 & 0.76 & 0.78 & 0.76 & 0.73 & 0.57 & 0.68 & \cellcolor[HTML]{CACDFA}\textbf{0.86} & 0.77 & 0.58 \\
\multirow{-4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mono-\\ Language\end{tabular}}} &  & \textit{M12} &  & 0.016 & 0.181 & \textbf{0.84} &  & 0.79 & \cellcolor[HTML]{CACDFA}\textbf{0.84} & \cellcolor[HTML]{CACDFA}\textbf{0.90} & \cellcolor[HTML]{CACDFA}\textbf{0.85} & \cellcolor[HTML]{CACDFA}\textbf{0.81} & 0.73 & \cellcolor[HTML]{CACDFA}\textbf{0.82} & \cellcolor[HTML]{CACDFA}\textbf{0.94} & \cellcolor[HTML]{CACDFA}{\color[HTML]{000000} \textbf{0.85}} & \cellcolor[HTML]{CACDFA}\textbf{0.83} \\ \hline
\end{tabular}
%%%%%%%%%%%%%%%%%%
}

{\footnotesize Erroneous \sip scores are in red. Confident \sip scores are in blue. Canonical Score serves as a baseline.}
\vspace{-0.15cm}

\end{table*}

==> tabs/results_2_correlations.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{\sip influence on Confounders and Deep Learning Error (bold: highest impact, shadowed: causal effect).}
\vspace{-0.2cm}
%\vspace{-0.1em}
\label{tab:correlations}

\scalebox{0.75}{

\setlength{\tabcolsep}{4pt} 

\begin{tabular}{lllrrrrrrrrlrrrr}
\hline
\multicolumn{2}{c}{\textbf{{[}T{]} Syntax Concepts}} &  & \multicolumn{8}{c}{\textbf{{[}Z{]} Code Confounders}} &  & \multicolumn{4}{c}{\textbf{{[}Y{]} DL Error}} \\ \cline{4-11}
\multicolumn{2}{c}{\textbf{}} &  & \multicolumn{2}{c}{\textbf{Cyclo Complexity}} & \multicolumn{2}{c}{\textbf{AST Levels}} & \multicolumn{2}{c}{\textbf{\# AST Nodes}} & \multicolumn{2}{c}{\textbf{Sequence Size}} &  & \multicolumn{4}{c}{\textbf{}} \\ \cline{4-11} \cline{13-16} 
\multicolumn{2}{c}{\textbf{}} &  & \multicolumn{1}{c}{\textbf{gpt-125}} & \multicolumn{1}{c}{\textbf{mono-2B}} & \multicolumn{1}{c}{\textbf{gpt-125}} & \multicolumn{1}{c}{\textbf{mono-2B}} & \multicolumn{1}{c}{\textbf{gpt-125}} & \multicolumn{1}{c}{\textbf{mono-2B}} & \multicolumn{1}{c}{\textbf{gpt-125}} & \multicolumn{1}{c}{\textbf{mono-2B}} &  & \multicolumn{2}{c}{\textbf{gpt-125}} & \multicolumn{2}{c}{\textbf{mono-2B}} \\ \cline{1-2} \cline{4-11} \cline{13-16} 
\multicolumn{1}{c}{\textbf{Category $\mathcal{C}$}} & \multicolumn{1}{c}{\textbf{$\alpha,\lambda$ nodes}} &  & \multicolumn{8}{c}{\textbf{rho}} &  & \multicolumn{1}{c}{\textbf{rho}} & \multicolumn{1}{c}{\textbf{ATE}} & \multicolumn{1}{c}{\textbf{rho}} & \multicolumn{1}{c}{\textbf{ATE}} \\ \hline
 & \textit{for\_statement} &  & 0.32 & 0.32 & 0.30 & 0.30 & 0.18 & 0.19 & 0.23 & 0.19 &  & -0.16 & \cellcolor[HTML]{EFEFEF}-0.10 & -0.07 & \cellcolor[HTML]{EFEFEF}-0.01 \\
\multirow{-2}{*}{\textit{\textbf{Iterative}}} & \textit{while\_statement} &  & 0.13 & 0.13 & 0.08 & 0.07 & 0.05 & 0.05 & 0.07 & 0.05 &  & -0.05 & \cellcolor[HTML]{EFEFEF}-0.11 & -0.03 & \cellcolor[HTML]{EFEFEF}-0.08 \\ \hline
 & \textit{identifier} &  & 0.10 & 0.12 & 0.10 & 0.20 & \textbf{0.51} & \textbf{0.46} & \textbf{0.49} & \textbf{0.49} &  & \textbf{-0.56} & \cellcolor[HTML]{EFEFEF}\textbf{-1.78} & \textbf{-0.80} & \cellcolor[HTML]{EFEFEF}\textbf{-2.89} \\
\multirow{-2}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Natural \\ Language\end{tabular}}}} & \textit{string} &  & 0.02 & 0.04 & 0.20 & 0.24 & 0.36 & 0.30 & 0.36 & 0.30 &  & -0.31 & \cellcolor[HTML]{EFEFEF}-0.36 & \textbf{-0.43} & \cellcolor[HTML]{EFEFEF}\textbf{-0.55} \\ \hline
 & \textit{return\_statement} &  & 0.27 & 0.14 & 0.06 & 0.28 & -0.06 & -0.03 & -0.01 & 0.32 &  & -0.04 & \cellcolor[HTML]{EFEFEF}-0.09 & -0.22 & \cellcolor[HTML]{EFEFEF}-0.09 \\
 & \textit{{]}} &  & 0.16 & 0.14 & 0.21 & 0.28 & 0.35 & 0.36 & 0.29 & 0.32 &  & -0.16 & \cellcolor[HTML]{EFEFEF}-0.04 & -0.22 & \cellcolor[HTML]{EFEFEF}-0.10 \\
\multirow{-3}{*}{\textit{\textbf{Scope}}} & \textit{)} &  & 0.09 & 0.03 & 0.07 & 0.12 & 0.37 & 0.23 & 0.31 & 0.23 &  & -0.37 & \cellcolor[HTML]{EFEFEF}-0.85 & \textbf{-0.54} & \cellcolor[HTML]{EFEFEF}\textbf{-1.49} \\ \hline
\textit{\textbf{Decision}} & \textit{if\_statement} &  & \textbf{0.58} & \textbf{0.58} & 0.29 & 0.28 & 0.20 & 0.21 & 0.27 & 0.23 &  & -0.22 & \cellcolor[HTML]{EFEFEF}-0.21 & -0.11 & \cellcolor[HTML]{EFEFEF}-0.11 \\ \hline
 & \textit{comparison\_operator} &  & 0.34 & 0.38 & 0.18 & 0.20 & 0.30 & 0.30 & 0.30 & 0.32 &  & -0.13 & \cellcolor[HTML]{EFEFEF}0.02 & -0.11 & \cellcolor[HTML]{EFEFEF}0.00 \\
\multirow{-2}{*}{\textit{\textbf{Operator}}} & \textit{boolean\_operator} &  & \textbf{0.53} & \textbf{0.54} & 0.20 & 0.21 & 0.17 & 0.18 & 0.22 & 0.20 &  & -0.10 & \cellcolor[HTML]{EFEFEF}0.01 & -0.08 & \cellcolor[HTML]{EFEFEF}-0.09 \\ \hline
 & \textit{for\_in\_clause} &  & 0.28 & 0.29 & 0.18 & 0.18 & 0.15 & 0.14 & 0.13 & 0.13 &  & -0.03 & \cellcolor[HTML]{EFEFEF}0.09 & -0.03 & \cellcolor[HTML]{EFEFEF}0.04 \\
 & \textit{if\_clause} &  & 0.20 & 0.22 & 0.10 & 0.10 & 0.06 & 0.06 & 0.07 & 0.06 &  & -0.01 & \cellcolor[HTML]{EFEFEF}0.19 & 0.01 & \cellcolor[HTML]{EFEFEF}0.13 \\
 & \textit{lambda} &  & -0.01 & -0.01 & 0.12 & 0.12 & 0.18 & 0.18 & 0.16 & 0.16 &  & -0.04 & \cellcolor[HTML]{EFEFEF}0.20 & -0.05 & \cellcolor[HTML]{EFEFEF}0.06 \\
\multirow{-4}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Functional \\ Programming\end{tabular}}}} & \textit{list\_comprehension} &  & 0.22 & 0.22 & 0.14 & 0.14 & 0.13 & 0.13 & 0.12 & 0.12 &  & -0.04 & \cellcolor[HTML]{EFEFEF}0.06 & -0.03 & \cellcolor[HTML]{EFEFEF}0.04 \\ \hline
\multicolumn{2}{c}{\textbf{Baseline}} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{1-2}
\textbf{Intrinsic} & Avg. Accuracy &  & \textbf{0.61} & \textbf{0.60} & \textbf{0.41} & \textbf{0.45} & \textbf{0.51} & \textbf{0.47} & \textbf{0.53} & \textbf{0.48} &  & -0.38 & \cellcolor[HTML]{EFEFEF}\textbf{-1.60} & -0.38 & \cellcolor[HTML]{EFEFEF}\textbf{-1.78} \\ \hline
\end{tabular}
} % % End Scalebox
\end{table*}


% % R1 - close to the ATE
% % R2 - close to the ATE
% % R3 - close to zero
% % R4 - close to the ATE


==> tabs/results_2_correlations_bk.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{\asccausal: Correlations and Causal Effects.}
\vspace{-0.1cm}
\label{tab:correlations}

\scalebox{0.85}{

\setlength{\tabcolsep}{4pt} 

\begin{tabular}{@{}ll|rrrrrrrr|rrrr@{}}
\toprule
\multicolumn{2}{c|}{\textbf{Variable}} &
  \multicolumn{2}{c}{\textbf{Cyclo Complexity}} &
  \multicolumn{2}{c}{\textbf{AST Levels}} &
  \multicolumn{2}{c}{\textbf{\# AST Nodes}} &
  \multicolumn{2}{c|}{\textbf{Sequence Size}} &
  \multicolumn{4}{c}{\textbf{Cross-Entropy Loss}} \\ \midrule
\multicolumn{2}{c|}{\textbf{LLMs}} &
  \multicolumn{1}{c}{\textbf{gpt-125}} &
  \multicolumn{1}{c}{\textbf{mono-2B}} &
  \multicolumn{1}{c}{\textbf{gpt-125}} &
  \multicolumn{1}{c}{\textbf{mono-2B}} &
  \multicolumn{1}{c}{\textbf{gpt-125}} &
  \multicolumn{1}{c}{\textbf{mono-2B}} &
  \multicolumn{1}{c}{\textbf{gpt-125}} &
  \multicolumn{1}{c|}{\textbf{mono-2B}} &
  \multicolumn{2}{c}{\textbf{gpt-125}} &
  \multicolumn{2}{c}{\textbf{mono-2B}} \\ \midrule
\multicolumn{1}{c}{\textbf{Category $\mathcal{H}$}} &
  \multicolumn{1}{c|}{\textbf{AsC}} &
  \multicolumn{8}{c|}{\textbf{$\rho = p(Y|T)$}} &
  \multicolumn{1}{c}{\textbf{$\rho$}} &
  \multicolumn{1}{c}{\textbf{Causal Eff.}} &
  \multicolumn{1}{c}{\textbf{$\rho$}} &
  \multicolumn{1}{c}{\textbf{Causal Eff.}} \\ \midrule
\textit{\textbf{Global}} &
  \textit{Avg. \asceval} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.61} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.60} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.41} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.45} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.51} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.47} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.53} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.48} &
  -0.38 &
  \cellcolor[HTML]{EFEFEF}\textbf{-1.60} &
  -0.38 &
  \cellcolor[HTML]{EFEFEF}\textbf{-1.78} \\ \midrule
 &
  \textit{for\_statement} &
  0.32 &
  0.32 &
  0.30 &
  0.30 &
  0.18 &
  0.19 &
  0.23 &
  0.19 &
  -0.16 &
  -0.10 &
  -0.07 &
  -0.01 \\
\multirow{-2}{*}{\textit{\textbf{Iterative}}} &
  \textit{while\_statement} &
  0.13 &
  0.13 &
  0.08 &
  0.07 &
  0.05 &
  0.05 &
  0.07 &
  0.05 &
  -0.05 &
  -0.11 &
  -0.03 &
  -0.08 \\ \midrule
 &
  \textit{identifier} &
  0.10 &
  0.12 &
  0.10 &
  0.20 &
  \cellcolor[HTML]{EFEFEF}\textbf{0.51} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.46} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.49} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.49} &
  \cellcolor[HTML]{EFEFEF}\textbf{-0.56} &
  \cellcolor[HTML]{EFEFEF}\textbf{-1.78} &
  \cellcolor[HTML]{EFEFEF}\textbf{-0.80} &
  \cellcolor[HTML]{EFEFEF}\textbf{-2.89} \\
\multirow{-2}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Natural \\ Language\end{tabular}}}} &
  \textit{string} &
  0.02 &
  0.04 &
  0.20 &
  0.24 &
  0.36 &
  0.30 &
  0.36 &
  0.30 &
  -0.31 &
  -0.36 &
  \cellcolor[HTML]{EFEFEF}\textbf{-0.43} &
  \cellcolor[HTML]{EFEFEF}\textbf{-0.55} \\ \midrule
 &
  \textit{return\_statement} &
  0.27 &
  0.14 &
  0.06 &
  0.28 &
  -0.06 &
  -0.03 &
  -0.01 &
  0.32 &
  -0.04 &
  -0.09 &
  -0.22 &
  -0.09 \\
 &
  \textit{{]}} &
  0.16 &
  0.14 &
  0.21 &
  0.28 &
  0.35 &
  0.36 &
  0.29 &
  0.32 &
  -0.16 &
  -0.04 &
  -0.22 &
  -0.10 \\
\multirow{-3}{*}{\textit{\textbf{Scope}}} &
  \textit{)} &
  0.09 &
  0.03 &
  0.07 &
  0.12 &
  0.37 &
  0.23 &
  0.31 &
  0.23 &
  -0.37 &
  -0.85 &
  \cellcolor[HTML]{EFEFEF}\textbf{-0.54} &
  \cellcolor[HTML]{EFEFEF}\textbf{-1.49} \\ \midrule
\textit{\textbf{Decision}} &
  \textit{if\_statement} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.58} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.58} &
  0.29 &
  0.28 &
  0.20 &
  0.21 &
  0.27 &
  0.23 &
  -0.22 &
  -0.21 &
  -0.11 &
  -0.11 \\ \midrule
 &
  \textit{comparison\_operator} &
  0.34 &
  0.38 &
  0.18 &
  0.20 &
  0.30 &
  0.30 &
  0.30 &
  0.32 &
  -0.13 &
  0.02 &
  -0.11 &
  0.00 \\
\multirow{-2}{*}{\textit{\textbf{Operator}}} &
  \textit{boolean\_operator} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.53} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.54} &
  0.20 &
  0.21 &
  0.17 &
  0.18 &
  0.22 &
  0.20 &
  -0.10 &
  0.01 &
  -0.08 &
  -0.09 \\ \midrule
 &
  \textit{for\_in\_clause} &
  0.28 &
  0.29 &
  0.18 &
  0.18 &
  0.15 &
  0.14 &
  0.13 &
  0.13 &
  -0.03 &
  0.09 &
  -0.03 &
  0.04 \\
 &
  \textit{if\_clause} &
  0.20 &
  0.22 &
  0.10 &
  0.10 &
  0.06 &
  0.06 &
  0.07 &
  0.06 &
  -0.01 &
  0.19 &
  0.01 &
  0.13 \\
 &
  \textit{lambda} &
  -0.01 &
  -0.01 &
  0.12 &
  0.12 &
  0.18 &
  0.18 &
  0.16 &
  0.16 &
  -0.04 &
  0.20 &
  -0.05 &
  0.06 \\
\multirow{-4}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Functional \\ Programming\end{tabular}}}} &
  \textit{list\_comprehension} &
  0.22 &
  0.22 &
  0.14 &
  0.14 &
  0.13 &
  0.13 &
  0.12 &
  0.12 &
  -0.04 &
  0.06 &
  -0.03 &
  0.04 \\ \bottomrule
\end{tabular}

} % % End Scalebox
\end{table*}


% % R1 - close to the ATE
% % R2 - close to the ATE
% % R3 - close to zero
% % R4 - close to the ATE


==> tabs/surveys.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\vspace{-0.1cm}
\begin{center}
\caption{User-Study Validity Results (bold: best agreement)}
\scalebox{0.80}{%

\setlength{\tabcolsep}{3pt} 

\begin{tabular}{lll|lccc}
\hline
\textbf{ID} &
  \textbf{Group} &
  \textbf{Description} &
  \multicolumn{4}{c}{\textit{\textbf{User study visualization results}}} \\ \hline
\textit{C} &
  \textit{Control} &
  \begin{tabular}[c]{@{}l@{}}Prompt\\ predicted tokens.\end{tabular} &
  \textbf{Agreement} &
  \textbf{\begin{tabular}[c]{@{}c@{}}\%\\ useful\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}\% \\ readable\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}\% \\ complex\end{tabular}} \\ \hline
\multirow{4}{*}{$S_1$} &
  \multirow{4}{*}{\textit{Sequence}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Prompt\\ predicted tokens\\ NTP.\end{tabular}} &
  Strongly &
  14 &
  0 &
  0 \\
 &
   &
   &
  Agree &
  \textbf{43} &
  29 &
  \textbf{43} \\
 &
   &
   &
  Neutral &
  29 &
  29 &
  29 \\
 &
   &
   &
  Disagree &
  14 &
  \textbf{43} &
  29 \\ \hline
\multirow{4}{*}{$S_2$} &
  \multirow{4}{*}{\textit{\begin{tabular}[c]{@{}l@{}}AST\\ partial\end{tabular}}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Prompt\\ predicted tokens\\ partial AST\\ NTP.\end{tabular}} &
  Strongly &
  14 &
  14 &
  0 \\
 &
   &
   &
  Agree &
  \textbf{29} &
  \textbf{43} &
  14 \\
 &
   &
   &
  Neutral &
  \textbf{29} &
  29 &
  \textbf{43} \\
 &
   &
   &
  Disagree &
  \textbf{29} &
  14* &
  \textbf{43} \\ \hline
\multirow{4}{*}{$S_3$} &
  \multirow{4}{*}{\textit{\begin{tabular}[c]{@{}l@{}}AST\\ complete\end{tabular}}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Prompt\\ predicted tokens\\ complete AST\\ NTP.\end{tabular}} &
  Strongly &
  0 &
  0 &
  17 \\
 &
   &
   &
  Agree &
  \textbf{50} &
  17 &
  \textbf{50} \\
 &
   &
   &
  Neutral &
  33 &
  33 &
  17 \\
 &
   &
   &
  Disagree &
  17 &
  \textbf{50} &
  17 \\ \hline
\end{tabular}
}%

\label{tab:survey}
\end{center}
{\footnotesize The * depicts the only \textit{``Strongly Disagree''} reported in the survey}
\end{table}

==> text/06.acknowledgment.tex <==
\section{Acknowledgments}
\label{sec:acknowledgments}

%This research has been supported in part by XXXX. We also acknowledge support from YYYY. Any opinions, findings, and conclusions expressed herein are the authors’ and do not necessarily reflect those of the sponsors. 
This research has been supported in part by NSF CCF-2311469, CCF-2007246, and CCF-1955853. We also acknowledge support from Cisco Systems. %Any opinions, findings, and conclusions expressed herein are the authors’ and do not necessarily reflect those of the sponsors. 

==> text/bk/03_experience_report.tex <==
\section{Experience Report}\label{sec:experience}

\DANIEL{This section should be completely rewritten and simplified, we just need to talk about the generated dataset and how we used it at galeras and astXplainer https://arxiv.org/pdf/2308.03873}
\subsection{Collecting Code Samples}
\input{tabs/dedupe}

As represented in the first step of the pipeline (refer to Fig.~\ref{fig:collection}-\circled{1}),  we filtered the most popular Python Github repositories using the following query: $language:Python$, $fork:false$, $size:>=30,000$,  $pushed:>2021-12-31$, $stars:>1,000$.

Our dataset aims to avoid data snooping, a problem where training samples are wrongly used to test statistical hypotheses. To do this, we focused on collecting code changes only up to January 2022. This is because we hypothesize \chatgpt and most newer \llms have not been trained on commits made after January 2, 2022, according to \cite{openai2023gpt4}. We carefully selected new methods from each commit, resulting in about 338K data points. For each of these data points, we extracted the comments or any associated documentation that describes its functionality.

In the second step (Fig.~\ref{fig:collection}-\circled{2}), we engineered and pre-processed code and documentation-related and security weaknesses from collected data points. We parsed the AST variables for our data points by employing the Tree-Sitter library. Therefore, each data point encompasses the \textit{code} and related features from the AST analysis. The AST features numerically describe the \ASTerrors, \ASTlevels, and \ASTnodes. The AST also describes the structural shape for the \textit{code} introducing the \textit{n\_words}, \textit{vocab\_size}, \tokenCount, and \whitespaces. The vocabulary size measures the count of unique words without repetition. \tokenCount is determined by using a universal tokenizer. We also calculated the number of variables that the \textit{code} is using and it is reflected as \identifiers. As for determining the security weaknesses, we use codeQL scanning suite \cite{noauthor_codeql_nodate}, focussing on the top `25'  Common Weakness Enumeration (CWE) \cite{noauthor_cwe_nodate}. CodeQL identifies vulnerability issues by scanning for predetermined rules defined with its query language. We report CodeQL results with the span positions of the identified vulnerability in the code. 

To guarantee efficient data management, we stored raw and preprocessed data points in a relational database once the previous features were engineered and extracted. Next, we removed duplicated samples using a distinct query reducing the testbed size to $\approx 227K$ data points for code. Of these reduced data points, $\approx 77K$ contains a valid \docstring. A \docstring is valid when its text is larger than 3 words. We use \textit{CLD3} library to detect the \textit{language} for each \docstring with a threshold of 0.9 to define sentence language such as English, Chinese, Spanish, etc.
Once these features were computed, the raw data was stored in a relational database, enabling efficient management and summarization of many data points.


In the third step \ref{fig:collection}-\circled{3}), we manually verified $960$ out of $\approx 227K$ data points. These verified data points were randomly selected from \textit{RawData} and \textit{RawDataDocstring} for a manual evaluation. The remaining data points underwent automatic validation. Our validation process ensures that the date of each pushed commit falls within the range of dates stated in the original query. Additionally, we confirmed that the methods associated with each commit were indeed updated within the same date range. Furthermore, we assessed the meaningfulness of the \docstring and \commitMessage by scrutinizing the consistency of the natural language descriptions with the actual code implementation, resulting in the removal of $\approx1.9\%$ from \textit{RawDataDocstring} and obtaining $\approx57K$ datapoints. Finally, \complexity was validated using the Codalyze plugin in Visual Studio Code.

In the final step (Fig.\ref{fig:collection}-\circled{4}), we sampled until $5k$ data points from the \textit{RawData} testbed to construct six additional testbeds, each tailored for a specific SE task. \snipgen encompasses \randomCut, \withDocstring, and \fromDocstring for \textit{code completion}; \commitGen for \textit{code generation}; \summarizationGen for \textit{code summarization}; and \textit{VulnerabilitySpan} for vulnerability detection. Details about these supplementary testbeds are outlined in Tab.~\ref{tab:dedupe}.

To create \randomCut, we selected data points with more than $10$ tokens or $100$ characters, and subsequently, each data point was randomly truncated after the method signature. For \summarizationGen and \commitGen, we filtered \textit{RawDataDocstring} data points with more than 10 words or 50 characters. After establishing the five testbeds, we employed Jaccard similarity on preprocessed data points with the BPE HuggingFace tokenizer to eliminate duplicate snippets. Given the absence of de-duplication between training and test sets (i.e., no multiset threshold), we configured a $0.7$ similarity threshold for our testbeds \cite{Allamanis19, wang_neural_2019}. Table.~\ref{tab:dedupe} provides information about the SE task associated with each curated testbed, the percentage of detected duplicates, final size and generated number of prompts.




 %Our methodology depicts data extraction based on experiment-specific parameters. Researchers are afforded the flexibility to choose datasets that align most seamlessly with their objectives. The pivotal role of \snipgen comes into play as it adeptly collects and extracts features from the chosen data. Each snippet is systematically labeled according to its relevance to a specific code generation sub-task in software engineering (SE). The presence of a \docstring within a snippet is leveraged by \snipgen to incorporate textual context seamlessly. Subsequently, a prompt template is strategically selected based on the SE sub-task, and a prompt is dynamically generated. This prompt serves as an invaluable tool for evaluating Language Model for Code (LLMc) but can also be efficiently trained and tested on canonical datasets, ensuring robustness and adaptability in the ever-evolving landscape of code generation research.




